Automated Tone Transcription and Clustering with Tone2Vec

Lexical tones play a crucial role in Sino-Tibetan languages. However, current phonetic fieldwork relies on manual effort, resulting in substantial time and financial costs. This is especially challenging for the numerous endangered languages that are rapidly disappearing, often compounded by limited funding. In this paper, we introduce pitch-based similarity representations for tone transcription, named Tone2Vec. Experiments on dialect clustering and variance show that Tone2Vec effectively captures fine-grained tone variation. Utilizing Tone2Vec, we develop the first automatic approach for tone transcription and clustering by presenting a novel representation transformation for transcriptions. Additionally, these algorithms are systematically integrated into an open-sourced and easy-to-use package, ToneLab, which facilitates automated fieldwork and cross-regional, cross-lexical analysis for tonal languages. Extensive experiments were conducted to demonstrate the effectiveness of our methods.

==> 050conclusion.tex <==
\section{Discussion}


\(\mathcal{M}\) not only automates tone transcription but yields hierarchical features for speech signals, laying the groundwork for automatic tone clustering across regions.



In response to the gap between machine learning and relational databases, we present ML Benchmark For Relational
Databases (RDBench). We provide hierarchical datasets and a user-friendly toolkit, offering various commonly used
data format interfaces: tabular data, homogeneous graph data, and heterogeneous graph data. It’s worth noticing that all
these data formats share an identical task definition. We also carried out extensive experiments on these datasets. With
the help of our unified task definition and easy-to-use interfaces, researchers from different ML subdomains can deploy
models, get comparable results and further enhance collaboration.
